Diffusion Convolutional Recurrent Neural Network: Data-Driven Traffic Forecasting

Spatiotemporal forecasting has various applications in neuroscience, climate and transportation domain. Traffic forecasting is one canonical example of such learning task. The task is challenging due to (1) complex spatial dependency on road networks, (2) non-linear temporal dynamics with changing road conditions and (3) inherent difficulty of long-term forecasting. To address these challenges, we propose to model the traffic flow as a diffusion process on a directed graph and introduce Diffusion Convolutional Recurrent Neural Network (DCRNN), a deep learning framework for traffic forecasting that incorporates both spatial and temporal dependency in the traffic flow. Specifically, DCRNN captures the spatial dependency using bidirectional random walks on the graph, and the temporal dependency using the encoder-decoder architecture with scheduled sampling. We evaluate the framework on two real-world large scale road network traffic datasets and observe consistent improvement of 12% - 15% over state-of-the-art baselines.

==> discussion.tex <==
Explain why explicitly model the graph structure improves the performance.

==> preliminaries.tex <==
\subsection{Structured Time Series Forecasting}
%
The goal of structured time series forecasting is to model the time series generated by a set of correlated objects\footnote{The correlation can be either spatial dependency, e.g., geospatial objects with correlation measured by distance, or topological dependency, e.g., follow/friend relationship in the social network. }
% We assume that either the spatial or topology dependency among objects is captured by the weighted directed graph.}, e.g., traffic sensors.
The pairwise relationship between those objects is modeled as a weighted directed graph
%a} structure, and we .
$\graph = (\vertices, \edges, \gweights)$, where $\vertices$ is a set of $\abs{\vertices} = N$ nodes, while $\edges$ is a set of edges and $\gweights{} \in \real^{N \times N}$ is a weighted adjacency matrix representing the proximity between nodes. 
$\M{D_O} = \mathrm{diag}(\M{W} \V{1})$ and $\M{D_I} = \mathrm{diag}(\M{W}^\intercal \V{1})$ denote the out-degree diagonal matrix and in-degree diagonal matrix respectively, where $\V{1}$ denotes the all one vector.
An observation of measurement on nodes at time $t$ can be viewed as a graph signal $\M{X}^{(t)}: \vertices \rightarrow \real^{d_X}$, where $d_X$ is the dimension of the signal at each node.

The structured time series forecasting problem can be formulated as follows:
% structured time series forecasting problem on a spatial graph.
given a graph $\graph$ and  $T'$ historical graph signals, infer the most likely graph signals in the next $T$ time steps:

\begin{equation}
    \M{\hat{X}}^{(t+T)}, \cdots, \M{\hat{X}}^{(t+1)} = 
    \underset{\M{X}^{(t+T)}, \cdots, \M{X}^{(t+1)}}{\arg\max } \log P(\M{X}^{(t+T)}, \cdots, \M{X}^{(t+1)} | \M{X}^{(t)},  \cdots, \M{X}^{(t-T'+1)}; \graph) \nonumber
\end{equation}
% Take traffic prediction for example, if each time step is 5 minutes and $H$ is 12, the outputs of the model will be the traffic of each sensor in every 5 minutes for the next hour.
%  i.e., $\M{X}^{(t+1)}, \cdots, \M{X}^{(t+T)}$, 
where $T'$ is the number of historical observations and $T$ is the forecasting horizon.
 
Many real-world problems can be formulated as the structured time series forecasting problem, including (1) traffic forecasting where the correlated objects are traffic sensors located on the road networks, and the time series are traffic flow;  (2) user activity modeling in social network where the correlated objects are users connected by the \textit{follow/friend} relationship in the social network graph, and time series are user activities at different times;  (3) power consumption/demand forecasting where the correlated objects are spatially correlated power stations and the time series are historical power consumptions.
% Note that the aforementioned structured time series forecasting problem is different from tasks defined in~\citet{xingjian2015convolutional} and~\citet{seo2016structured}.
% The prediction target of our problem is a sequence of multivariate time series distributed over a weighted or unweighted directed or undirected graph $\graph$.
It is also worth mentioning that tasks defined in~\citet{xingjian2015convolutional} and~\citet{seo2016structured} can be considered as special cases of this problem where $\graph$ is either a regular grid, e.g., an image, or an undirected graph.

\subsection{Graph Random Walk and Personalized Page Rank}
% \todo{See something about the random walk process}.
Given a graph $\graph = (\vertices, \edges, \gweights)$, and a starting node $v_i \in \vertices$, we select one of its neighbors, e.g., $v_j$, with probability proportional to $W_{ij}$, and move to $v_j$; then we select a neighbor of $v_j$ and continue this process. The random sequence of points selected this way is a \textit{random walk} on the graph. 
Random walk also defines a Markov chain with transition matrix $\M{D}_O^{-1}\M{W}$.
Suppose $\V{\pi}^{(t)}$ is the distribution on the graph, with $\pi^{(t)}_i$ represents the probability of being at $v_i$ at time $t$. The distribution after one step random walk $\V{\pi}^{(t+1)} = \left(\M{D}_O^{-1}\M{W}\right)^\intercal \V{\pi}^{(t)}$.

Personalized Page Rank (PPR)~\citep{haveliwala2003ppr} is an important method to estimate the relevance of nodes imposed by the graph structure.
% \footnote{More explanation about Personalized Page Rank can be found in the supplemental material.}
Suppose, $\alpha \in [0, 1]$ is the restarting probability in the random walk process, the personalized page rank matrix $\M{\ppr} \in \real^{N\times N}$ is a transition matrix whose $i$th row $\V{\ppr}_{i, :} \in \real{}^N$ represents the stationary distribution of the random walk that restarts at $v_i \in \vertices$ with probability $\alpha$.
Larger value in $\V{\ppr}_{i, :}$ roughly means greater relevance with respects to $v_i$.
% \todo{Explain more about PPR, PPR is a way to model the topological relevance of nodes in a graph}
Specifically, PPR can be represented as a weighted combination of infinite random walks on the graph, and be calculated in closed form using Equation~\ref{eq:ppr}~\citep{teng2016scalable}:
\begin{equation}
% \V{p}_u = \alpha \V{1}_u + (1-\alpha) \M{W}^\intercal \M{D}_O^{-1} \V{p}_u
\M{\ppr} = \alpha \M{I} + \sum_{k=1}^\infty  \alpha(1-\alpha) ^k \left(\M{D}_O^{-1} \M{W} \right)^k
\label{eq:ppr}
\end{equation}
% Later, we show that 
% \todo{See PPR and Random Walk can be used to model spatial dependency}


% $\alpha\sum_{k=0}^\infty(1-\alpha)^k=1$, and 
% where $\M{D}_O^{-1}\M{W}$ is the transition matrix of random walk, and $\M{\ppr}$ can be considered as a

% The filter centered as each node are represented using weights from the PPR.
